Unbiased Gradient Estimation for Distributionally Robust Learning

Seeking to improve model generalization, we consider a new approach based on distributionally robust learning (DRL) that applies stochastic gradient descent to the outer minimization problem. Our algorithm efficiently estimates the gradient of the inner maximization problem through multi-level Monte Carlo randomization. Leveraging theoretical results that shed light on why standard gradient estimators fail, we establish the optimal parameterization of the gradient estimators of our approach that balances a fundamental tradeoff between computation time and statistical variance. Numerical experiments demonstrate that our DRL approach yields significant benefits over previous work.

==> algo_progressive.tex <==

\section{Algorithm and Analysis} \label{sec:algo}
%
%, defined more precisely below, includes a (slight) generalization of the bisection-search result in \cite{nd16,nd17} for
%the inner maximization problem by utilizing similar results in~\cite{gl18} for $KL$-divergences and showing that this approach can be
%successfully applied to other $\phi$-divergence metrics.
%The computational effort is still of order $O(M\log M)$ for $D_{\chi^2}$-constraints and of order $O(M)$ for $D_{KL}$-constraints where $M$
%is the dimension of the decision variables, in our case the size of the dataset support of the pmf.
%Hence, instead of operating with the complete dataset $M_t=N$ for all iterations $t$ of a full-gradient descent algorithm, we propose the
%following stochastic subgradient descent scheme
\refalg{alg:overall} presents our dynamically sampled subgradient descent algorithm for efficiently solving general min-max optimization problems.
The algorithm follows SGD-like iterations for the outer minimization problem in~\eqref{absfmln}:
\begin{equation}\label{ssgd}
\theta_{t+1} = \theta_t - \gamma_t \nabla_{\theta} \hat{R}_{t}(\theta_t), 
\end{equation}
where $\gamma_t$ is
%known as
the step size (or gain sequence or learning rate) and $\hat{R}_{t}(\cdot)$ is a stochastic approximation of the robust loss $R(\cdot)$ from the
inner maximization formulation over $D_{\phi}$-constrained $\cP$.
This view of~\eqref{absfmln} allows us to depart from the convex-concave formulations of~\citeN{bhwmg13} and consider non-convex losses $l$,
as long as $\nabla_{\theta} \hat{R}_{t}(\cdot)$ approximates the gradient $\nabla_{\theta} {R}(\cdot)$ sufficiently well.
The existence of $\nabla_{\theta} R(\theta)$ is given by Danskin's Theorem (Theorem 7.21, pg.~352 of ~\citeN{shap09}) along with our assumptions
in ~\refthm{thm:bias} to ensure a unique optimum for the inner maximization.
We depart from~\citeN{nd16} and \citeN{nd17} in that we construct the estimate $\hat{R}_t$ by solving the inner maximization problem restricted
only to a relatively small subset $\cM_t$ of the full dataset with size $|\cM_t| = M_t$.
In particular, the subset ${\cM_t}$ is constructed by {\em uniformly} sampling {\em without replacement} $M_t$ values from the complete training
dataset (of size $N$).
Sampling without replacement differs from the standard with-replacement approach in the stochastic optimization literature, though it is preferred
by practitioners in machine/deep learning.
\refrem{rmk:smpl} below describes why this strategy is needed here.

%Defining $\hat{P} = (\hat{p}_m)$
Defining ${P} = ({p}_m)$
of dimension $M_t$ and the objective coefficients $z_m = l(\theta,\xi_m)$, we have 
\begin{align} \label{restrob}
&\hat{R}_{t}(\theta) \quad=\quad \max_{{P}=({p}_m)} \sum_{m\in\cM_t}{p}_m z_m \\
&\mbox{s.t. }  \sum_{m\in\cM_t} \phi(M_t {p}_m) \le M_t\rho_{t},\, \, \sum_{m\in\cM_t} {p}_m = 1 ,\, {p}_m \ge 0. \nonumber
\end{align}
Here the constraint parameter $\rho_t$ now changes with $t$; see~\refthm{thm:bias} (\refsec{ssec:ssapx}).
Further note that $\phi$-divergence metrics
%are strong in that they can only
assess distances between probability measures defined on the same support,
%. This limits our study of (6) to considering only 
and thus \eqref{restrob} considers
subsampling from discrete distributions
%and
which
is the primary motivation for using the corresponding tools of probability.
%Wasserstein distances are weaker metrics in that they can provide a finite value for distances between discrete and continuous distributions, and so the tools used in that case to study (6) must allow for feasibility of arbitrary distributions.

Now suppose ${P}_t^*(\theta) = ({p}^*_{t,m}(\theta))$ is an optimal solution to~\eqref{restrob}.
Then a valid subgradient for $\hat{R}_t(\theta_t)$ is obtained from 
\begin{equation}
\nabla_{\theta} \hat{R}_{t}(\theta_t) \quad=\quad
\sum_{m\in\cM_t}{p}^*_{t,m}(\theta_t) \,\,\,\,\nabla_{\theta} l(\theta_t,\xi_m).
\label{subprob:grad}
\end{equation}
This expression for the gradient estimator follows from the same arguments that lead to the form of the full gradient $\nabla_{\theta} R(\theta)$ provided by Danskin's Theorem,
which establishes the validity of this gradient expression for optimization problems meeting certain criteria that is satisfied by our inner-maximization problem (see~\refprop{prop:props}).
%The reviewer is correct about this seemingly counter-intuitive result.
%This expression for the gradient arises from applying Danskin’s theorem,
%which is a deep result that shows the validity of this gradient expression
%for optimization problems that meet certain criteria (as does our inner-max problem).
\refthm{thm:bias} provides a bound on the error in using \eqref{subprob:grad} to approximate $\nabla_{\theta}{R}$ (the gradient of the true full-sample robust loss) as a function of the sample size $M_t$.
This bound on the bias vanishes only as $M_t\nearrow N$ as $t\tndi$.
Since fixed bias violates a basic requirement for SGD that the gradient estimator
$\E[\nabla\hat{R}_t(\theta)] = \Theta(\nabla R(\theta))$\footnote{We use standard
time complexity notation; see~\citeN{sipser06}.}
%(see Section~4.3 in \citeN{bcn16}),
(see \citep[Section~4.3]{bcn16}),
then the convergence of \eqref{ssgd} cannot be guaranteed when $M_t=M,\,\forall t$ where $M<N$.
%We were using the standard big-Theta  notation bounding a function from above and below. Specifically, two sequences are a_n = \Theta(b_n) if there exist constants c, d such that c \le \lim_n (a_n/b_n) \le d. 

\citet[Theorem 4.7]{bcn16} show that diminishing step-sizes are used in standard SGD ($M_t=M$)
%in order
to eliminate the impact of noise when gradient estimators are unbiased.
\citet[Section 5.1]{bcn16} further show that keeping step-sizes fixed and increasing the estimation mini-batch size directly is more advantageous (informally) because larger
$M_t$ in later iterations makes the gradient estimates more accurate.
In our case, the SGD algorithm~\eqref{ssgd} requires sample size growth even to eliminate bias, and this also provides decrease in noise as a consequence.
The maximum size $N$ is hit after a (large) finite number of iterations $T$, at which point it is advisable to switch to a deterministic optimization algorithm,
e.g.,~\citeN{nd17}.

When increasing $M_t$, it is no longer necessary to diminish the step size $\gamma_t$;
indeed, doing so negates the benefits of the extra work in computing gradients using
larger $M_t$. 
% For strongly convex functions, Theorem 6 shows that the best balance between the extra work to obtain more accurate estimates and the faster convergence afforded by strong convexity is struck by growing $M_t$ geometrically, similar to Theorem 5.1 in [3]. [15,A2] analogously analyze convex and non-convex functions but the results are less striking; informally, they conclude that since full-batch deterministic iterates exhibit slower than linear convergence, the $M_t$ may grow slower than geometric but the overall work complexity convergence is also slower than in the strongly convex case.
%We are extending our analysis along these lines.
%
%
%Another important consequence of progressively increasing $M_t$ is that it also reduces the variance (or noise) in the gradient estimate, and a decreasing gain sequence $\gamma_t$ is no longer needed to offset the impact of noise.
\refalg{alg:overall} therefore takes large fixed-length steps $\gamma$.
\refthm{thm:main-gen} shows that our algorithm gets substantially close in performance to $R_{\inf}$ in $T$ iterations when the sample set sizes $M_t$ are chosen to satisfy a
%certain
minimum-growth condition.
The analysis applies to the case where $l(\theta,\xi)$ possess Lipschitz gradients but may otherwise be non-convex.
This allows our algorithm to be used in important cases when $l(\cdot,\xi_n)$ are non-convex, such as training deep learning models. 
%
\begin{algorithm}[!htp]
	\caption{Dynamically Sampled Subgradient Descent}\label{alg:overall}
	{\bf Given}: Step size $\gamma$;~
	Sample size sequence $\{M_t\}_{t=1}^T$, $M_T=N$;
	Initial iterate $\theta_0$.
%; Set $T = \log(N/M_0) / (-\log(\nu))$.
	\begin{algorithmic}[1]
		% \Algphase{Estimation}
		\FOR { $t=1,2,\ldots,T$}
		\STATE\label{step:enstart} 
		Sample $M_t$ indices {\em without replacement} uniformly from
		$\{1,\ldots,N\}$, and gather them in $\cM_t$ %  {\em unique} indices \Comment{$|\cM_t |\le M_t$}
		\STATE Solve inner maximization problem to obtain optimal solution ${P}^*_{t}\qquad$
		\COMMENT{see \refsec{ssec:robopt}}
		% \State Sample a set $\cS_t$ of $M_t$ indices i.i.d. from $\{1,\ldots,N\}$ using pmf
		% $P^*_{\cM_t}$ 
		\STATE Set $G_t \gets \sum_{m\in\cM_t} {p}^*_{t,m} \nabla l(\theta_t,\xi_m)$
		\STATE Set $\theta_{t+1} \gets \theta_t - \gamma G_t \quad$
		\COMMENT{subgradient descent step}
		%\STATE Set $M_{t+1} \gets M_t\,\,/\,\,\nu $
		\STATE Increment $t\gets t+1$
		\ENDFOR
	\end{algorithmic}
\end{algorithm}

Further addressed below is the question of choosing a {\em good} value for the step-length $\gamma$ and the sample growth sequence that obtains an optimal balance
between the added computational burden of each iteration and the expected reduction in the optimality gap.
We show for the case of strong-convex loss functions $l(\theta,\xi)$ that too slow a growth sequence, namely diminishing-factor growth (defined below), is inefficient,
while constant-factor growth sequences are efficient in the sense that the expected optimality gap drops at a rate proportional to the increase in the computational effort.
Extending these results to the convex and non-convex cases are subjects
%of focus
of our ongoing research.

Our detailed analysis starts with an estimation of the effort needed to obtain an
exact solution to the inner maximization problem, followed by two subsections establishing
various mathematical properties for our approach w.r.t.\ bias and convergence, respectively,
thus providing theoretical justification for the settings in our algorithm.
The following additional notation is used extensively: For a sequence of positive-valued
random variables (r.v.s) $\{A_n\}$, we write $A_n=o_p(1)$ if $A_n \inP 0$ as $n \to \infty$;
We write $A_n=\mathcal{O}_p(1)$ if $\{A_n\}$ is stochastically bounded, that is, for a given $\epsilon>0$
there exists $c(\epsilon) \in (0,\infty)$ with $\mathbb{P}(A_n < c(\epsilon)) > 1 - \epsilon$
for sufficiently large $n$;
If $\{B_n\}$ is another sequence of positive-valued r.v.s, we write $A_n = \mathcal{O}_p(B_n)$ if $A_n/B_n= \mathcal{O}_p(1)$. 


\input{inner_max}
\input{bias}
\input{convergence}

